Longitudinal Wrist PPG Analysis for Reliable Hypertension Risk Screening Using Deep Learning

Hypertension is a leading risk factor for cardiovascular diseases. Traditional blood pressure monitoring methods are cumbersome and inadequate for continuous tracking, prompting the development of PPG-based cuffless blood pressure monitoring wearables. This study leverages deep learning models, including ResNet and Transformer, to analyze wrist PPG data collected with a smartwatch for efficient hypertension risk screening, eliminating the need for handcrafted PPG features. Using the Home Blood Pressure Monitoring (HBPM) longitudinal dataset of 448 subjects and five-fold cross-validation, our model was trained on over 68k spot-check instances from 358 subjects and tested on real-world continuous recordings of 90 subjects. The compact ResNet model with 0.124M parameters performed significantly better than traditional machine learning methods, demonstrating its effectiveness in distinguishing between healthy and abnormal cases in real-world scenarios.

==> main.tex <==

@inproceedings{sarkar2020self,
  title={Self-supervised learning for ecg-based emotion recognition},
  author={Sarkar, Pritam and Etemad, Ali},
  booktitle={ICASSP 2020-2020 IEEE International Conference on Acoustics, Speech and Signal Processing (ICASSP)},
  pages={3217--3221},
  year={2020},
  organization={IEEE}
}

@inproceedings{vardhan2021bp,
  title={BP-Net: Efficient deep learning for continuous arterial blood pressure estimation using photoplethysmogram},
  author={Vardhan, K Rishi and Vedanth, S and Poojah, G and Abhishek, K and Kumar, M Nitish and Vijayaraghavan, Vineeth},
  booktitle={2021 20th IEEE International Conference on Machine Learning and Applications (ICMLA)},
  pages={1495--1500},
  year={2021},
  organization={IEEE}
}
@inproceedings{schlesinger2020blood,
  title={Blood pressure estimation from PPG signals using convolutional neural networks and Siamese network},
  author={Schlesinger, Oded and Vigderhouse, Nitai and Eytan, Danny and Moshe, Yair},
  booktitle={ICASSP 2020-2020 IEEE international conference on acoustics, speech and signal processing (ICASSP)},
  pages={1135--1139},
  year={2020},
  organization={IEEE}
}
@inproceedings{truong2022non,
  title={Non-invasive blood pressure monitoring with multi-modal in-ear sensing},
  author={Truong, Hoang and Montanari, Alessandro and Kawsar, Fahim},
  booktitle={ICASSP 2022-2022 IEEE International Conference on Acoustics, Speech and Signal Processing (ICASSP)},
  pages={6--10},
  year={2022},
  organization={IEEE}
}
@inproceedings{suhas2024end,
  title={End-To-End Personalized Cuff-Less Blood Pressure Monitoring Using ECG and PPG Signals},
  author={Suhas, BN and Srinivasa, Rakshith Sharma and Saidutta, Yashas Malur and Cho, Jaejin and Lee, Ching-Hua and Yang, Chouchang and Shen, Yilin and Jin, Hongxia},
  booktitle={ICASSP 2024-2024 IEEE International Conference on Acoustics, Speech and Signal Processing (ICASSP)},
  pages={2101--2105},
  year={2024},
  organization={IEEE}
}
@inproceedings{tian2020cross,
  title={Cross-domain joint dictionary learning for ECG reconstruction from PPG},
  author={Tian, Xin and Zhu, Qiang and Li, Yuenan and Wu, Min},
  booktitle={ICASSP 2020-2020 IEEE International Conference on Acoustics, Speech and Signal Processing (ICASSP)},
  pages={936--940},
  year={2020},
  organization={IEEE}
}
@inproceedings{he2016deep,
  title={Deep residual learning for image recognition},
  author={He, Kaiming and Zhang, Xiangyu and Ren, Shaoqing and Sun, Jian},
  booktitle={Proceedings of the IEEE conference on computer vision and pattern recognition},
  pages={770--778},
  year={2016}
}

@misc{who_hypertension,
  author       = {{World Health Organization}},
  title        = {Hypertension},
  howpublished = {\textit{WHO}},
  url          = {https://www.who.int/news-room/fact-sheets/detail/hypertension},
  note         = {Accessed: 29-Aug-2024}
}
@article{vaswani2017attention,
  title={Attention is all you need},
  author={Vaswani, A},
  journal={Advances in Neural Information Processing Systems},
  year={2017}
}
@article{paviglianiti2022comparison,
  title={A comparison of deep learning techniques for arterial blood pressure prediction},
  author={Paviglianiti, Annunziata and Randazzo, Vincenzo and Villata, Stefano and Cirrincione, Giansalvo and Pasero, Eros},
  journal={Cognitive Computation},
  volume={14},
  number={5},
  pages={1689--1710},
  year={2022},
  publisher={Springer}
}
@article{van2016wavenet,
  title={Wavenet: A generative model for raw audio},
  author={Van Den Oord, Aaron and Dieleman, Sander and Zen, Heiga and Simonyan, Karen and Vinyals, Oriol and Graves, Alex and Kalchbrenner, Nal and Senior, Andrew and Kavukcuoglu, Koray and others},
  journal={arXiv preprint arXiv:1609.03499},
  volume={12},
  year={2016}
}
@article{qin2023cuff,
  title={Cuff-less blood pressure prediction based on photoplethysmography and modified ResNet},
  author={Qin, Caijie and Li, Yong and Liu, Chibiao and Ma, Xibo},
  journal={Bioengineering},
  volume={10},
  number={4},
  pages={400},
  year={2023},
  publisher={MDPI}
}
@article{johnson2016mimic,
  title={MIMIC-III, a freely accessible critical care database},
  author={Johnson, Alistair EW and Pollard, Tom J and Shen, Lu and Lehman, Li-wei H and Feng, Mengling and Ghassemi, Mohammad and Moody, Benjamin and Szolovits, Peter and Anthony Celi, Leo and Mark, Roger G},
  journal={Scientific data},
  volume={3},
  number={1},
  pages={1--9},
  year={2016},
  publisher={Nature Publishing Group}
}
@article{wang2023pulsedb,
  title={PulseDB: A large, cleaned dataset based on MIMIC-III and VitalDB for benchmarking cuff-less blood pressure estimation methods},
  author={Wang, Weinan and Mohseni, Pedram and Kilgore, Kevin L and Najafizadeh, Laleh},
  journal={Frontiers in Digital Health},
  volume={4},
  pages={1090854},
  year={2023},
  publisher={Frontiers Media SA}
}
@ARTICLE{10360188,
  author={Ma, Chenbin and Sun, Yangyang and Zhang, Peng and Song, Fan and Feng, Youdan and He, Yufang and Zhang, Guanglei},
  journal={IEEE Transactions on Instrumentation and Measurement}, 
  title={SMART-BP: SEM-ResNet and Auto-Regressor Based on a Two-Stage Framework for Noninvasive Blood Pressure Measurement}, 
  year={2024},
  volume={73},
  number={},
  pages={1-18},
  keywords={Predictive models;Feature extraction;Statistics;Sociology;Prediction algorithms;Monitoring;Pipelines;Automatic machine learning;blood pressure (BP) waveform;deep learning;photoplethysmography (PPG);two-stage},
  doi={10.1109/TIM.2023.3342856}}
@article{he2022new,
  title={A new approach for daily life Blood-Pressure estimation using smart watch},
  author={He, Jiayu and Ou, Jianlin and He, An and Shu, Lin and Liu, Tao and Qu, Ruowen and Xu, Xiangmin and Chen, Zhuoming and Yan, Yifeng},
  journal={Biomedical Signal Processing and Control},
  volume={75},
  pages={103616},
  year={2022},
  publisher={Elsevier}
}
@article{cho2014learning,
  title={Learning phrase representations using RNN encoder-decoder for statistical machine translation},
  author={Cho, Kyunghyun and Van Merrienboer, Bart and Gulcehre, Caglar and Bahdanau, Dzmitry and Bougares, Fethi and Schwenk, Holger and Bengio, Yoshua},
  journal={arXiv preprint arXiv:1406.1078},
  year={2014}
}
@article{abbaspourazad2023large,
  title={Large-scale training of foundation models for wearable biosignals},
  author={Abbaspourazad, Salar and Elachqar, Oussama and Miller, Andrew C and Emrani, Saba and Nallasamy, Udhyakumar and Shapiro, Ian},
  journal={arXiv preprint arXiv:2312.05409},
  year={2023}
}

@misc{AHA2024,
  title        = {Understanding Blood Pressure Readings},
  author       = {{American Heart Association}},
  year         = 2024,
  url          = {https://www.heart.org/en/health-topics/high-blood-pressure/understanding-blood-pressure-readings},
  note         = {Accessed: 2024-09-06}
}
@inproceedings{vraka2023harnessing,
  title={Harnessing Photoplethysmography and Deep Learning in Continuous Blood Pressure Monitoring for Early Hypertension Detection},
  author={Vraka, Aikaterini and Hornero, Fernando and F{\'a}cila, Lorenzo and Ravelli, Flavia and Alcaraz, Ra{\'u}l and Rieta, Jos{\'e} J},
  booktitle={International Conference on e-Health and Bioengineering},
  pages={213--220},
  year={2023},
  organization={Springer}
}

